Private-Yet-Verifiable Contact Tracing

We propose PrYVeCT, a private-yet-verifiable contact tracing system. PrYVeCT works also as an authorization framework allowing for the definition of fine-grained policies, which a certain facility can define and apply to better model its own access rules. Users are authorized to access the facility only when they exhibit a contact trace that complies with the policy. The policy evaluation process is carried out without disclosing the personal data of the user. At the same time, each user can prove to a third party (e.g., a public authority) that she received a certain authorization. PrYVeCT takes advantage of oblivious automata evaluation to implement a privacy-preserving policy enforcement mechanism.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

==> motivating.tex <==
\subsection{Motivating scenario}
\label{sec:example}

Consider the following scenario. The education authority wants to properly manage the physical accesses to the classrooms.
On the one hand they would like to maximize the number of students in a classroom. On the other hand, they want to keep the risk of contagion under a certain threshold. 

As already mentioned in the introduction, the education authority may establish a quarantine policy, whereby  all students deemed at risk of developing the infection (possibly because they recently met with someone who was later declared infectious)  must connect from remote. In this case, our system should allocate authorization tokens only to those who are considered not at risk of developing the infection.

However, if the benefit of attending classes in person is very large, the  education authority may wish to implement a more permissive policy, for example one that allows at most $n$ ``at risk students'' in the same classroom, where $n$ is a parameter.  Given this policy, our system should allocate authorization tokens   to at most $n$ ``risky'' students  (as well as to all those deemed not risky). Note that if $n=0$ we are back to the quarantine policy described above.

Clearly, if $n>0$ such policy has a global scope w.r.t. the entire group of people that can access the classroom, i.e., the students. Thus, it cannot be (locally) enforced on a single individual, but can only be enforced on the entire group. Said differently, whereas when $n=0$  each user receives an authorization token independently on whether other users also receive an authorization token, this is not the case when $n>0$.

%Clearly, the policy defined above has a global scope w.r.t. the entire group of people that can access the classroom, i.e., the students. Thus, it cannot be (locally) enforced on a single individual. Said differently, the enforcement authority needs to process the private information of all the individuals. % A further aspect is the expressive power of the policy language. As a matter of fact, characterizing the \emph{potentially risky contacts} requires a predicate to be evaluated over the contact trace. Such a predicate can be non trivial as it may depend on parameters such as time or geographical location of the individuals.
